The braid group surjects onto $G_2$ tensor space

Let V be the 7-dimensional irreducible representation of the quantum group U_q(g_2). For each n, there is a map from the braid group B_n to the endomorphism algebra of the n-th tensor power of V, given by R-matrices. We can extend this linearly to a map on the braid group algebra. Lehrer and Zhang (MR2271576) prove this map is surjective, as a special case of a more general result. Using Kuperberg's spider for G_2 from arXiv:math.QA/9201302, we give an elementary diagrammatic proof of this result.

==> documentclasshack.tex <==
%auto-ignore
%%%%%% a hack to make the documentclass name available later %%%
% Thanks to Morten Høgholm. I stole this code from 
% http://groups.google.com/group/comp.text.tex/msg/142306cc7f8acdac
\let\LaTeXdocumentclass\documentclass
\renewcommand*\documentclass[2][]{%
   \newcommand*\ClassName{#2}% for later use
   \LaTeXdocumentclass[#1]{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> todolist.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
\section*{todo list}
\begin{enumerate}
\item Write this todo list.
\end{enumerate}


==> xypdf-c.tex <==
%% xypdf-c.tex from $Id: xypdf-c.doc,v $
%%
%% Xy-pic ``Colour extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-cloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-cloaded\endcsname=\empty \xycatcodes
\expandafter\ifx \csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\UsePDFcolor{\installPDFcolor@}
\xydef@\NoPDFcolor{\UnloadColor@}
\xydef@\installPDFcolor@{\installPDFstyle@
 \let\xymath@=\xyPDFmath@ \let\xynomath@=\xyPDFnomath@
 \let\checkxyPDFcolor@=\checkxyPDFcolor@@
 \let\xycolor@@=\xyPDFcolor@@
 \xystandardcolors@ 
 \xyuncatcodes }
\xydef@\xyPDFmath@{\hbox\bgroup\dimen@=.55ex \checkxyPDFcolor@ \xyinside@}
\xydef@\xyPDFnomath@{\hbox\bgroup\dimen@=\z@ \checkxyPDFcolor@ \xyinside@}
\xydef@\checkxyPDFcolor@@{\edef\pdfsaved@color{\pdfcurrent@color}%
 \let\checkxyPDFcolor@=\relax}
\xylet@\checkxyPDFcolor@=\relax
\xydef@\xyPDFnewcolor@#1#2#3#4#5{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@\newxycolor{#1}{}\relax\fi
 \DNii@{#4}\ifx\nextii@\empty
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPDFcolor@{#2//#3}}\else
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPDFcolor@{#4}}\fi
 \ifx\nextii@\empty\expandafter\def\next@{\xyPDFnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}\expandafter\tmp@\fi }
\xylet@\newxycolor@=\xyPDFnewcolor@
\xydef@\xyPDFcolor@{\ifPDFspecials@\expandafter\xyPDFcolor@@
 \else\expandafter\eat@\fi}
\xydef@\xyPDFcolor@@#1{\bgroup \checkXyStyle@ 
 \def\preStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPDFpre@}}%
 \def\postStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPDFpost@}}%
 \let\modPDFboxz@=\modXYstyle@ \xyPDF@color@@{#1}%
 \toks@={\egroup\let\xy@style@=\relax \def\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Drop@@}\def\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Connect@@}}%
 \the\toks@ }

\xydef@\pdfcurrent@color{1 1 1 1 k 1 1 1 1 K}
\xydef@\pdfsaved@color{1 1 1 1 k 1 1 1 1 K}
\xydef@\xyPDF@color@@#1{%
 \edef\pdfsaved@color{\pdfcurrent@color}%
 \pdf@convertcolor#1////!%
 \edef\next@{\noexpand\xyPDFsplitPDF@{\pdfcurrent@color}{\pdfsaved@color}}%
 \next@}
\xydef@\pdf@convertcolor#1//#2//#3!{\DN@{#2}%
 \DNii@{cmyk}\ifx\next@\nextii@\DN@{#1 k #1 K}%
 \else \DNii@{rgb}\ifx\next@\nextii@\DN@{#1 rg #1 RG}%
 \else \DNii@{gray}\ifx\next@\nextii@\DN@{#1 #1 #1 rg #1 #1 #1 RG}%
 \else \DN@{1 1 1 1 k 1 1 1 1 K}%
 \fi \fi \fi 
 \expandafter\def\expandafter\pdfcurrent@color\expandafter{\next@}}
\xydef@\xycolor@raw@@#1{}%
\endinput


==> xypdf-f.tex <==
%% xypdf-f.tex from $Id: xypdf-f.doc,v $
%%
%% Xy-pic ``Frame extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-floaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-floaded\endcsname=\empty \xycatcodes
\xydef@\installPDFframes@{%
 \let\framed@body@@=\xyPDFframed@body@
 \let\circled@x@@=\xyPDFcircled@x@
 \let\ellipsed@x@@=\xyPDFellipsed@x@
 \installPDFfills@
 \xyuncatcodes}
\xydef@\UsePDFframes{\installPDFframes@}
\xydef@\NoPDFframes{\UnloadFrames@}
\xydef@\xyPDFframed@body@{\DN@{\framed@body@}%
 \ifx\framehfill\frm@solidh@@
 \DN@{\xyPDFframed@oval@\xyPDFoval@Special}%
 \else\ifdim\R@=\z@\else
 \ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFframed@oval@\xyPDFdashoval@Special}%
 \else\ifx\framehfill\frm@doth@@
 \DN@{\xyPDFframed@oval@\xyPDFdotoval@Special}%
 \fi\fi
 \fi\fi \next@ }
\xydef@\xyPDFframed@oval@#1{\vglue\U@c
 \hbox{\hglue\L@c\xypdfoval@#1\hglue\R@c}\vglue\D@c}
\xydef@\xyPDFcircled@x@{\DN@{\xyPDFcircled@x@@\xyPDFcirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPDFcircled@x@@\xyPDFdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFcircled@x@@\xyPDFdashcirc@Special}%
 \fi\fi \next@ }
\xydef@\xyPDFcircled@x@@#1{\vglue2\R@
 \hbox{\hglue2\R@\xypdfcircle@#1\hglue2\R@}%
 \vglue2\R@}
\xydef@\xyPDFellipsed@x@#1#2{%
 \DN@{\xyPDFellipsed@x@@\xyPDFcirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPDFellipsed@x@@\xyPDFdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFellipsed@x@@\xyPDFdashcirc@Special}%
 \fi\fi \next@{#1}{#2}}
\xydef@\xyPDFellipsed@x@@#1#2#3{\vglue #3\vglue #3\relax
 \hbox{\L@c = #2\relax \R@c=\L@c \D@c = #3\relax \U@c=\D@c 
 \hglue#2\hglue#2\relax\xypdfellipse@#1\hglue#2\hglue#2\relax}%
 \vglue #3\vglue #3\relax}
\xydef@\xyPDFdashhfill@{{\SemiDirectionChar=95 \Direction=3072 \xyPDFdash@}}
\xydef@\xyPDFdashvfill@{{\SemiDirection=31 \Direction=1023 \xyPDFdash@}}
\xydef@\xypdfoval@#1{%
 \dimen@=\L@c \advance\dimen@\R@c
 \dimen@ii=\U@c \advance\dimen@ii\D@c 
 \ifdim\dimen@ii<\dimen@ \relax \dimen@=\dimen@ii\fi \divide\dimen@\tw@
 \ifdim\R@>\dimen@ \relax \R@=\dimen@ \fi
 \D@c=-\D@c \L@c=-\L@c 
 \edef\tmp@{\expandafter\removePT@\the\R@
 \space\expandafter\removePT@\the\R@c 
 \space\expandafter\removePT@\the\D@c 
 \space\expandafter\removePT@\the\L@c 
 \space\expandafter\removePT@\the\U@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypdfcircle@#1{\dimen@=\R@
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypdfellipse@#1{\edef\tmp@{%
 \expandafter\removePT@\the\U@c \space
 \expandafter\removePT@\the\D@c \space
 \expandafter\removePT@\the\L@c \space
 \expandafter\removePT@\the\R@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xyPDFoval@Special#1{\PDFmacro@{#1 ov}}%%%%<<<---- here
\xydef@\xyPDFcirc@Special#1{\PDFmacro@{#1 ox}}%%%%<<<---- here
\xydef@\xyPDFdotcirc@Special#1{\PDFmacro@{#1 ot}}%%%%<<<---- here
\xydef@\xyPDFdashcirc@Special#1{\PDFmacro@{#1 od}}%%%%<<<---- here
\xydef@\xyPDFdotoval@Special#1{\PDFmacro@{#1 vt}}%%%%<<<---- here
\xydef@\xyPDFdashoval@Special#1{\PDFmacro@{#1 vd}}%%%%<<<---- here
\xydef@\xyPDFfilledRegion#1#2{\setboxz@h{\lower\D@c\vbox{%
 \vglue\U@c\hbox{#1#2\empty\hglue\L@c\hglue\R@c}\vglue\D@c}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\filledRectangle@PDF{%
 \xyPDFfilledRegion{\xypdfoval@\xyPDFfilloval@Special}}
\xydef@\filledCircle@PDF#1{{\R@c=\R@ \L@c=\R@ \U@c=\R@ \D@c=\R@
 \xyPDFfilledRegion{\xypdfcircle@\xyPDFfillcirc@Special}#1}}
\xydef@\filledEllipse@PDF{%
 \xyPDFfilledRegion{\xypdfellipse@\xyPDFfillellipse@Special}}
\xydef@\filledOval@PDF{%
 \xyPDFfilledRegion{\xypdfoval@\xyPDFfilloval@Special}}
\xydef@\frame@emph@PDF#1{\filled@{#1}\relax}
\xydef@\installPDFfills@{%
 \let\frame@emph@@=\frame@emph@PDF
 \let\filledRectangle@@=\filledRectangle@PDF
 \let\filledOval@@=\filledOval@PDF
 \let\filledCircle@@=\filledCircle@PDF
 \let\filledEllipse@@=\filledEllipse@PDF
}
\xydef@\xyPDFfilloval@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfo}%%%%%<<<---- here
 \else\PDFmacro@{#1 fo}\fi}%%%%<<<---- here
\xydef@\xyPDFfillcirc@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfc}%%%%%<<<---- here
 \else\PDFmacro@{#1 fc}\fi}%%%%<<<---- here
\xydef@\xyPDFfillellipse@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfe}%%%%%<<<---- here
 \else\PDFmacro@{#1 fe}\fi}%%%%<<<---- here
\endinput


==> xypdf-l.tex <==
%% xypdf-l.tex from $Id: xypdf-l.doc,v $
%%
%% Xy-pic ``Line extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-lloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-lloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\installPDFline@{\installPDFstyle@
 \installPDFlinestyles@ \installPDFpolylines@ }
\xydef@\UsePDFlines{\installPDFline@}
\xydef@\NoPDFlines{\UnloadLine@\relax}
\xydef@\xyPDFlineSpecial@#1{\xyPDFrawZ@{ #1 w}}
\xydef@\xyPDFcapSpecial@#1{\xyPDFrawZ@{ #1 J}}
\xydef@\xyPDFjoinSpecial@#1{\xyPDFrawZ@{ #1 j}}
\xydef@\xyPDFmiterSpecial@#1{\xyPDFrawZ@{ #1 M}}
\xydef@\installPDFlinestyles@{%
 \let\xylinewidth@@=\xylinewidth@
 \let\transxyline@@=\transxyline@
 \let\xylineSpecial@@=\xyPDFlineSpecial@
 \let\resetxyline@@=\resetxyline@i
 \let\xy@linecap@@=\xy@linecap@
 \let\xycapSpecial@@=\xyPDFcapSpecial@
 \let\resetxylinecap@@=\resetxylinecap@i
 \let\xy@linejoin@@=\xy@linejoin@
 \let\xyjoinSpecial@@=\xyPDFjoinSpecial@
 \let\resetxylinejoin@@=\resetxylinejoin@i
 \let\xy@linemiter@@=\xy@linemiter@
 \let\xymiterSpecial@@=\xyPDFmiterSpecial@
 \let\resetxylinemiter@@=\resetxylinemiter@i
}
\xydef@\xypolylinePDF@Special#1{\PDFspecial@@{ q [] 0 d #1 S Q}}
\xydef@\xypolydotPDF@Special#1{\PDFspecial@@{ q [1 3] 0 d S Q}}
\xydef@\xypolydashPDF@Special#1{\PDFspecial@@{ q [5] 0 d #1 S Q}}
\xydef@\xypolyfillPDF@Special#1{\PDFspecial@@{ q #1 f Q}}
\xydef@\xypolyeofillPDF@Special#1{\PDFmacro@{ q #1 f* Q}}
\xydef@\installPDFpolylines@{%
 \let\xypolyline@Special=\xypolylinePDF@Special
 \let\xypolydot@Special=\xypolydotPDF@Special
 \let\xypolydash@Special=\xypolydashPDF@Special
 \let\xypolyfill@Special=\xypolyfillPDF@Special
%\let\xypolyeofill@Special=\xypolyeofillPDF@Special
 \let\xy@polystyle@@=\xy@polystyle@ }
\endinput


==> xypdf-r.tex <==
%% xypdf-r.tex from $Id: xypdf-r.doc,v $
%%
%% Xy-pic ``PDF Rotations and Scaling''.
%% Copyright (c) 1999-1999 Ross Moore <ross@maths.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-rloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-rloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\installPDFrotscale@{\installPDFstyle@
% \let\xyRotate@@=\xyPDFrotate@@
% \let\doSpecialRotate@@=\doPDFspecialRotate@@
 \let\xyscale@@=\xyPDFscale@@
 \xyPDFshapes@true
 \xyuncatcodes }
\xydef@\UsePDFrotate{\installPDFrotscale@}
\xydef@\NoPDFrotate{\UnloadRotate@\relax}
\xydef@\xyPDFpretransform@{\xyPDFrawA@{\preXYtransform@@}}
\xydef@\xyPDFposttransform@{\xyPDFrawZ@{\postXYtransform@@}}
\let\preXYtransform@=\xyPDFpretransform@
\let\postXYtransform@=\xyPDFposttransform@
\xydef@\xyPDFrotSplit@{%
 \expandafter\def\expandafter\preShape@@\expandafter{\xyPDFpre@}%
 \expandafter\def\expandafter\postShape@@\expandafter{\xyPDFpost@}}
\xydef@\xyPDFscale@@#1#2{%
 \xyPDFsplitPDF@{\xyscale@start(#1,#2)}{\xyscale@end}%
 \xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\xyPDFrotate@@#1{%
 \xyPDFsplitPDF@{\xyrot@start(#1 xyd)}{\xyrot@end}%%%<<------ here
 \xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\xyPDFspecialRotate@#1{%
 \xyPDFsplitPDF@{\xyrot@start(#1)}{\xyrot@end}\xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\doPDFspecialRotate@@#1@@{\xyPDFspecialRotate@{#1}}
\xydef@\xyRotScale@@{%
% \def\xyrot@start(##1){{xyt ##1\space xyr}}%%%<<------ here
 \def\xyscale@start(##1,##2){ q ##1 0 0 ##2 0 0 cm}%
 \def\xyrot@end{ Q}\def\xyscale@end{ Q}}
\endinput


==> xypdf-s.tex <==
%% xypdf-s.tex from $Id: xypdf-s.doc,v $
%%
%% Xy-pic ``Style extension'' PDF support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-sloaded\endcsname=\empty \xycatcodes
\xydef@\xykillstyles@@{\Unloadstyle@}%
\xywarnifdefined\xyPDFescapestyle@
\xywarnifdefined\xyPDFsplitescape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPDFescapestyle@#1@@{\xyPDFsplitescape@#1<><>@@}%
 \gdef\xyPDFsplitescape@#1<>#2<>#3@@{\xyescape@@{#1}{#2}}}
\xydef@\xyPDFsplitPDF@#1#2{%
 \def\xyPDFpre@{#1}\def\xyPDFpost@{#2}\modPDFboxz@ }
\xydef@\xyescape@@#1#2{\checkXyStyle@ 
 \applyFIFOstyle@\prexyescape@{#1}\postxyescape@{#2}}
\xydef@\prexyescape@{\xyescapeSpecial@}
\xydef@\postxyescape@{\xyescapeSpecial@}
\xylet@\xyescapeSpecial@=\eat@
\let\xyescapeSpecial@=\addtostyletoks@
\xydef@\installPDFstyle@{%
 \def\preXYstyle@@{\xyPDFpre@}%
 \let\xydoprestyles@=\xyPDFrawstyleA@
 \let\xydopoststyles@=\xyPDFrawZ@
 \let\xykillstyles@=\xykillstyles@@
 }
\xydef@\xyPDFrawstyleA@#1{\xyPDFrawA@{{#1}{}}}
\endinput


==> xypdfpdf.tex <==
%% xypdfpdf.tex from $Id: xypdfpdf.doc,v $
%%
%% Xy-pic ``PDF-PDF'' PDF support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-pdfloaded\endcsname=\empty \xycatcodes
\global\newif\ifPDFspecials@
\xylet@\PDFmacro@@=\eat@
\xylet@\PDFdict@@=\eat@
\xylet@\PDFspecial@@=\eat@
\xylet@\PDFread@@=\eat@
\xylet@\PDFinclude@@=\eat@
\xylet@\PDFraw@@=\eat@
\xylet@\xyPDFobeylines@@=\relax
\xylet@\PDFspecialdict@@=\eat@
\xydef@\UnloadPDFpdf@{%
 \let\PDFmacro@@=\eat@
 \let\PDFdict@@=\eat@
 \let\PDFspecial@@=\eat@
 \let\PDFread@@=\eat@
 \let\PDFinclude@@=\eat@
 \let\PDFraw@@=\eat@
 \let\xyPDFobeylines@@=\relax
 \let\PDFspecialdict@@=\eat@
}
\xydef@\UnloadPDF@{\UnloadPDFpdf@
 \expandafter\ifx\csname xypdfloaded\endcsname\unknown\PDFspecials@false
 \else\expandafter\NoPDFspecials\fi}
\xylet@\UnloadPDF@@=\UnloadPDF@
\ifx\undefined\dvitype@\xydef@\dvitype@{null}\fi
\xylet@\xyrealshipout@=\shipout
\xydef@\xyPDFshipout@{\xyrealshipout@}
\xydef@\firstPDF@{%
 \global\let\firstPDF@@=\relax \global\let\firstPDF@=\relax}
\xylet@\firstPDF@@=\firstPDF@
\xylet@\dumpPDFdict@@=\relax
\xydef@\installxypdf@{%
 \xyinputorelse@{xypdfpdf}{\xydrivernoload@{pdfpdf}}\xycatcodes
 \installxypdf@@ \installxypdf@x }
\xylet@\installxypdf@@=\relax
\xylet@\setupxyPDF@@=\PDFspecials@true
\xywithoption{pdf}{\let\setupxyPDF@@=\setupxyPDF@}
\xydef@\installxypdf@x{
 \let\firstPDF@=\relax
 \let\XYpredict@=\relax
 \setupxyPDF@@ }
\xydef@\setupxyPDF@{\PDFspecials@true}
\let\realinstallxypdf@x=\installxypdf@x
\ifx\undefined\AfterBeginDocument
 \def\installxypdf@x{\xysetup@@{\realinstallxypdf@x}}%
\else
 \def\installxypdf@x{\AfterBeginDocument{\realinstallxypdf@x}}%
\fi
\xydef@\xydefaultdriver@{dvipdf}
\xydef@\xyPDFdriver#1{\def\xydefaultdriver@{#1}}
\xydef@\installxypdf@orig{\DN@{}%
 \ifx\xydriversselected@@\empty
 \DN@{\expandafter\defaultinstallpdf@\expandafter{\xydefaultdriver@}}%
 \else \def\do##1{%
 \expandafter\ifx\csname##1@xy@pdf\endcsname\relax
 \DN@{\defaultinstallpdf@{##1}}}%
 \xydriversselected@@ 
 \else \DN@##1{}\fi\fi \next@ }
\xydef@\defaultinstallpdf@#1#2{%
 \xywarning@{no driver specified, using #1 }%
 \xyrequire{#1}\csname #1@xy@pdf\endcsname{}}
\xydef@\null@xy@pdf{\installxypdf@}
\xydefcsname@{shape [!...]}#1{%
 \expandafter\ifx\csname xypdf-sloaded\endcsname\empty \DN@{\xyPDFescapestyle@{#1}@@}%
 \else\ifxyPDFshapes@\DN@{\xyPDFshapechar@{#1}@@}%
 \else \DN@{\xyPDFcharwarning@}\fi\fi \next@ }
\xydefcsname@{shape [pdfxy]}{\ifxyPDFshapes@\DN@{\xyPDFpdfxy@}%
 \else \DN@{\xyPDFcharwarning@}\fi \next@ }
\xydef@\xyPDFpdfxy@{%
 \setboxz@h{\dimen@=\L@p \advance\dimen@-\R@p 
 \dimen@ii=-\U@p \raise\dimen@ii\hbox to\z@{%
 \kern\dimen@\xyPDFcurrpt@\kern-\dimen@}\boxz@}}%
\xydef@\xyPDFcurrpt@{\ifxyPDFshapes@\expandafter\xyPDFcurrpt@@\fi}
\xydef@\xyPDFcurrpt@@@{\PDFspecial@@{xyi}\PDFraw@@{userdict begin xyx end}}%%%%<<<<<--- here
\ifx\undefined\xyPDFcurrpt@@ \xylet@\xyPDFcurrpt@@=\xyPDFcurrpt@@@ \fi
\xywarnifdefined\xyPDFshapechar@
\xywarnifdefined\xyPDFsplitshape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPDFshapechar@#1@@{\xyPDFsplitshape@#1<><>@@}%
 \gdef\xyPDFsplitshape@#1<>#2<>#3@@{\xyPDFsplitPDF@{#1}{#2}}}
\xydef@\xyPDFrawA@#1{\expandafter\xyPDFrawAA@ #1{}{}}%
\xydef@\xyPDFrawAA@#1#2{\PDFraw@@{ #1 #2}\PDFmessage{ #1 #2 }}%
\xydef@\xyPDFrawZ@#1{\PDFraw@@{ #1}\PDFmessage{ #1 }}%
\xydef@\modPDFboxz@{%
 \expandafter\DN@\expandafter{\xyPDFpre@{}}\ifx\next@\empty\else
 \setboxz@h{\expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}\boxz@
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}\DN@{}\fi}%
\xydef@\modPDFdrop@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Drop@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}%
 \DN@##1{\expandafter\def\expandafter\Drop@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\modPDFconnect@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Connect@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}%
 \DN@##1{\expandafter\def\expandafter\Connect@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\xyPDFpre@{{}{}}
\xydef@\xyPDFpost@{}
\xydef@\PDFmessage@#1{\W@{PDF: #1}}
\xydef@\PDFignore@#1{}%
\xydef@\showPDFmessages{\let\PDFmessage=\PDFmessage@}
\xydef@\hidePDFmessages{\let\PDFmessage=\PDFignore@}
\xylet@\PDFtracing=\showPDFmessages
\hidePDFmessages
\xydef@\PDFmacro@#1{\PDFmacro@@{#1}\PDFmessage{#1}}
\xydef@\includeXYPDFdict@{\relax}
\xydef@\xyPDFdictknown@{}
\xywarnifdefined\obeyoutlines@
{\catcode`\^^M=\active%
 \gdef\obeyoutlines@{\catcode`\^^M=\active \def^^M{^^J}%
 \newlinechar=`\^^J\obeyspaces}}
\xynew@{if}\ifxyPDFshapes@ \xyPDFshapes@true 
\xydef@\xyPDFcharwarning@@{\xyPDFcharmessage@
 \gdef\xyPDFcharwarning@@{\xyPDFcharmessage@
 \xywarning@{...no further PDF warnings will be given}%
 \global\let\xyPDFcharwarning@@=\relax }}
\xydef@\xyPDFcharmessage@{\xywarning@{%
 the current <driver> does not fully support PDF effects}}%
\xydef@\newxyshape#1#2#3{%
 \DN@{#3}\ifx\next@\empty
 \xydefcsname@{shape [#1]}{\csname xyshape@#1@\endcsname}%
 \else \expandafter\def\csname shape [#1]\endcsname{%
 \csname xyshape@#1@\endcsname}\fi
 \DN@{#2}\ifx\next@\empty
 \expandafter\def\csname xyshape@#1@\endcsname{%
 \xyundefinedEffect@{#1}{}@@}%
 \else \expandafter\def\csname xyshape@#1@\endcsname{#2}\fi }
\xydef@\xyundefinedEffect@#1#2@@{%
 \xywarning@{The #1 #2 effect is not implemented with the current driver}}%
\xydef@\newxyPDFshape#1#2{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@ \newxyshape{#1}{}\relax\fi
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{#2}%
 \ifx\nextii@\empty\expandafter\def\next@{\xyPDFnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}%
 \expandafter\tmp@\fi }
\xydef@\xyPDFnotimplemented@@#1@@{%
 \xywarning@{This PostScript effect is not implemented yet}}%
\xydef@\xyPDFnotfinished@@{%
 \xywarning@{This effect is not reliable yet; box sizes may be wrong}}%
\installxypdf@
\endinput








==> xypdftex.tex <==
%% xypdftex.tex from $Id: xypdftex.doc,v $
%%
%% Xy-pic ``pdf-TeX'' driver interface option.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{pdftex}{pdf-TeX driver}{\stripRCS$Revision: 3.8 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\pdfTeX@@#1{\dvimessage@{pdf-TeX}{#1}}
\newdriver{%
 \xyaddsupport{color}\pdftexColor@@
 \xyaddsupport{crayon}\pdftexCrayon@@
% \xyaddsupport{pdf}\pdftexPDF@@
% \xyaddsupport{rotate}\pdftexRotate@@
 \xyaddsupport{line}\pdftexLine@@
% \xyaddsupport{frame}\pdftexFrames@@
% \xyaddsupport{tile}\pdftexTiles@@
 \xyaddsupport{cmtip}\relax
}
%\xydef@\pdfTeXcolor@push#1{\special{pdfcolor push}\special{pdfcolor #1}}
\xydef@\pdfTeXcolor@push#1{\edef\pdfsaved@color{\pdfcurrent@color}%
 \def\pdfcurrent@color{#1}\special{#1}}%%%<<<<<<--- WRONG !
\xydef@\pdfTeXcolor@pop{\let\pdfcurrent@color\pdfsaved@color
 \expandafter\special\expandafter{\pdfsaved@color}}
\xydef@\pdfTeXcolours@{\pdftexPDFtypes@
% \let\xylocalColor@=\xystackcolor@
% \let\xycolor@push=\pdfTeXcolor@push
% \let\xycolor@pop=\pdfTeXcolor@pop
 \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-c}{\xydrivernoload@{pdf-c}}%
 \if@pdf@known\installPDFcolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\pdftexCrayon@@{}}%
 \else\let\next@=\xystandardcolors@ \fi \next@ 
 \let\xycolorwarning@=\relax \pdfTeX@@{color}%
 \let\pdftexColor@@=\relax
 \let\UnloadColor@@=\NopdfTeXcolor@
 }
\xydef@\pdftexColor@@{\pdfTeXcolours@}
\xydef@\NopdfTeXcolor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\pdftexColor@@=\pdfTeXcolours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\pdftexCrayon@@{\pdftexColor@@\pdftexCrayon@}
\xydef@\pdftexCrayon@{\installCrayolaColors@}%
\xydef@\pdftexPDF@@{\if@pdf@known\pdftexPDF@}
\xydef@\pdftexPDFunload@{\if@pdf@known\UnloadPDF@
 \let\UnloadPDF@@=\UnloadPDF@
 \let\pdftexPDF@@=\pdftexPDF@ }
\xydef@\pdftexPDFtypes@{%
 \xyinputorelse@{xypdfpdf}{\xydrivernoload@{pdfpdf}}%
 \ifx\PDFspecial@@\pdfTeXspecial@\else
 \let\PDFspecial@@=\pdfTeXspecial@
 \let\PDFmacro@@=\pdfTeXmacro@
 \let\PDFdict@@=\pdfTeXdict@
 \let\PDFraw@@=\pdfTeXraw@
 \let\PDFinclude@@=\pdfTeXinclude@
 \let\PDFspecialdict@@=\pdfTeXspecialDict@
 \let\xyPDFobeylines@@=\obeypdfTeXlines@
 \pdfTeX@@{PDF}%
 \fi \pdftexCurrpt@ }
\xydef@\pdfTeXspecial@#1{\if@pdf@known\firstPDF@@\pdfobj{#1}\pdflastobj}
\xydef@\pdfTeXmacro@#1{\pdfobj{#1}}
\xydef@\pdfTeXdict@#1{\pdfnames{#1}}
\xydef@\pdfTeXspecialDict@#1{\pdfnames{#1}}
\xydef@\pdfTeXinclude@#1{\if@pdf@known\firstPDF@@\special{prePDFfile #1}}
\xydef@\pdfTeXraw@#1{\if@pdf@known\firstPDF@@\pdfliteral{#1}}%
{\catcode`\^^M=\active%
 \gdef\next{\catcode`\^^M=\active \let^^M=\par%
 \let\PDFspecial@@=\pdfTeXdict@ \obeyspaces}}
\xylet@\obeypdfTeXlines@=\next
\xydef@\pdftexCurrpt@{\let\xyPDFcurrpt@@=\pdftexCurrpt@@}%
\xydef@\pdftexCurrpt@@{\PDFspecial@@{xyi}\PDFraw@@{userdict begin xyx end}}%%%%%<<<<<--- here
\xydef@\pdftexPDF@{\pdftexPDFtypes@
 \let\pdftexPDF@@=\relax
 \let\UnloadPDF@@=\pdftexPDFunload@ 
 \let\installxypdf@@=\relax \if@pdf@known\installxypdf@ }
\xydef@\pdftexRotate@@{\pdftexRotate@}
\xydef@\pdftexRotate@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-r}{\xydrivernoload@{pdf-r}}%
 \xyRotScale@@ \if@pdf@known\installPDFrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}\if@pdf@known\UnloadRotate@\relax}\fi
 \next@}
\xydef@\pdftexLine@@{\pdftexLine@}
\xydef@\pdftexLine@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-l}{\xydrivernoload@{pdf-l}}%
 \if@pdf@known\installPDFline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\if@pdf@known\UnloadLine@\relax}\fi
 \next@ }
\xydef@\pdftexFrames@@{\pdftexFrames@}
\xydef@\pdftexFrames@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-f}{\xydrivernoload@{pdf-f}}%
 \if@pdf@known\installPDFframes@ }%
 \else\DN@{\xydriverfail@{frames are}\if@pdf@known\UnloadPDFframes@\relax}\fi
 \next@ }
\xydef@\pdftexTiles@@{\pdftexTiles@}
\xydef@\pdftexTiles@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-t}{\xydrivernoload@{pdf-t}}%
 \if@pdf@known\installPDFpatterns@ \xystandardpatterns@}%
 \else\DN@{\xydriverfail@{Patterns are}\if@pdf@known\UnloadPDFpatterns@\relax}\fi
 \next@ }
\xydef@\if@pdf@known#1{\ifx\undefined#1\else\expandafter#1\fi}
\xyendinput



